Global Perspectives of AI Risks and Harms: Analyzing the Negative Impacts of AI Technologies as Prioritized by News Media

Emerging AI technologies have the potential to drive economic growth and innovation but can also pose significant risks to society. To mitigate these risks, governments, companies, and researchers have contributed regulatory frameworks, risk assessment approaches, and safety benchmarks, but these can lack nuance when considered in global deployment contexts. One way to understand these nuances is by looking at how the media reports on AI, as news media has a substantial influence on what negative impacts of AI are discussed in the public sphere and which impacts are deemed important. In this work, we analyze a broad and diverse sample of global news media spanning 27 countries across Asia, Africa, Europe, Middle East, North America, and Oceania to gain valuable insights into the risks and harms of AI technologies as reported and prioritized across media outlets in different countries. This approach reveals a skewed prioritization of Societal Risks followed by Legal & Rights-related Risks, Content Safety Risks, Cognitive Risks, Existential Risks, and Environmental Risks, as reflected in the prevalence of these risk categories in the news coverage of different nations. Furthermore, it highlights how the distribution of such concerns varies based on the political bias of news outlets, underscoring the political nature of AI risk assessment processes and public opinion. By incorporating views from various regions and political orientations for assessing the risks and harms of AI, this work presents stakeholders, such as AI developers and policy makers, with insights into the AI risks categories prioritized in the public sphere. These insights may guide the development of more inclusive, safe, and responsible AI technologies that address the diverse concerns and needs across the world.

==> definitions-of-risk-categories.tex <==
\textit{AI governance risks} - this category describes the regulatory risks associated to policies and regulations proposed or set by governments or corporations that may hinder the development, deployment, and licensing of AI technologies such as over-regulating or under-regulating the use of AI. For example, one risks of over-regulating AI is ``..potentially hinder[ing] European companies like Germany's Aleph Alpha or France's Mistral AI from competing globally." In contrast, an example of under-regulating the use of AI  in the U.S. is: ``United States regulators have fallen short of the tough approach European governments have taken on tech regulation and in crafting strong rules on deepfakes and misinformation.

technologies . information risks, existential risks, user experience risks, ethical risks, humanness risks, structure \& power risks, mental \& emotional risks, AI performance risks, environmental risks, safety risks, risks pertaining to the authoritative use of AI, over-reliance risks, technology adoption risks, disruption of service risks, and media risks

